Dynamic Ridesharing in Peak Travel Periods

In this paper, we study a variant of the dynamic ridesharing problem with a specific focus on peak hours: Given a set of drivers and rider requests, we aim to match drivers to each rider request by achieving two objectives: maximizing the served rate and minimizing the total additional distance, subject to a series of spatio-temporal constraints. Our problem can be distinguished from existing work in three aspects: (1) Previous work did not fully explore the impact of peak travel periods where the number of rider requests is much greater than the number of available drivers. (2) Existing solutions usually rely on single objective optimization techniques, such as minimizing the total travel cost. (3) When evaluating the overall system performance, the runtime spent on updating drivers' trip schedules as per incoming rider requests should be incorporated, while it is excluded by most existing solutions. We propose an index structure together with a set of pruning rules and an efficient algorithm to include new riders into drivers' existing trip schedule. To answer new rider requests effectively, we propose two algorithms that match drivers with rider requests. Finally, we perform extensive experiments on a large-scale test collection to validate the proposed methods.

==> alg-divideconquer.tex <==
\setlength{\algomargin}{1.2em} 
\begin{smaller}
	\begin{algorithm}  
		\caption{ The Divide-and-conquire Algorithm (DC) }   
		\label{dc:main}   
		\begin{algorithmic}[1] %"1" represents that it will show number in each row  
			\REQUIRE  %Input  
			a driver set $D$, a rider request set $R$, a threshold $\gamma$
			\ENSURE  %Output  
			subgraphs each of which consisting of driver-and-rider pairs;  
			\IF {Size($R$) $\leq \gamma$}										\label{dc:if}
			\STATE solve problem ($D$, $R$) to get the result directly			
			\ELSE
			\STATE divide ($D$, $R$) into ($D_1$, $R_1$) and ($D_2$, $R_2$)
			\STATE execute $DC (D_1, R_1)$ to get answer $S_1$
			\STATE execute $DC (D_2, R_2)$ to get answer $S_2$
			\STATE merge ($S_1$, $S_2$) to get the result $S$
			\ENDIF
		\end{algorithmic}  
	\end{algorithm}
\end{smaller}

==> alg-relaxationbaseline.tex <==
\setlength{\algomargin}{1.2em} 
\begin{smaller}
\begin{algorithm}[htb]   
	\caption{ Relaxation Baseline Algorithm (RB) }   
	\label{relaxationbaseline}   
	\begin{algorithmic}[1] %"1" represents that it will show number in each row  
		\REQUIRE  %Input  
		a driver set $D$, an unserved rider request $r$, waiting constraint step \waitrelax, detour constraint step \detourrelax, maximal iteration time \iteration
		\ENSURE  %Output  
		return a suitable driver $d$
		\STATE \augdistance$\leftarrow 0$, \optaugdistance$\leftarrow\infty$, $d^*\leftarrow NIL$, \optntripschedule$\leftarrow NIL$, $w^\prime$=$w$+\waitrelax$\times$(\iteration/2), $\theta^\prime$=\detour+\detourrelax$\times$(\iteration/2)  \label{ba:initial}	
		\FOR {$d \in D$}																				\label{ba:for:start}
		\IF[Definition 5 (3)]{\dist($d$,$r$) $\leq$ $w^\prime$}  		
		\FOR {$i \leftarrow$\sarr[$d.id$] \TO $n$} 								 \label{ba:for:for:start}
		\STATE initialize $at$, $lt$, $sl$, and $cp$ using Eq. \ref{equ:at}-Eq. \ref{equ:cp}
		\IF[Definition 5 (1)(4)] {$cp[i]\textless n$ or \detourdis($o_i$,\source,$o_{i+1}$)$\textgreater sl[i+1]$} 			
		\CONTINUE														   	\label{ba:for:for:if}
		\ENDIF	
		\FOR {$j \leftarrow$\darr[$d.id$] \TO $n$}														    
		\IF[Definition 5 (2)(5)(6)] {$cp[j]\textless n$ or \dist(\source,$o_{i+1}$)+\dist($o_{i+1},o_j$)+\dist($o_j$, \des))$\textgreater$(1+$\theta^\prime$)\dist(\source,\des) or \detourdis($o_j$,\source,$o_{j+1}$)$\textgreater sl[j+1]$} 				\label{ba:for:for:for:if}
		\CONTINUE					
		\ENDIF
		\STATE \optntripschedule $\leftarrow$ insert \source and \des at $i$-th and $j$-th location in $d.$\tripschedule		
		\STATE \augdistance $\leftarrow$compute the augmented travel distance using Equation \ref{augdistance} based on \optntripschedule	 		\label{ba:for:for:for:compute}
		\IF { \augdistance $\textless$ \optaugdistance }												\label{ba:for:for:for:compare}
		\STATE \optaugdistance $\leftarrow$ \augdistance, $d^* \leftarrow d$							\label{ba:for:for:for:update}
		\ENDIF
		\ENDFOR	
		\ENDFOR
		\ENDIF
		\ENDFOR 
		\RETURN $d^*$
	\end{algorithmic}  
\end{algorithm} 
\end{smaller}








==> alg-relaxationopt.tex <==
\setlength{\algomargin}{1.2em} 
\begin{smaller}
\begin{algorithm}[htb]   
	\caption{ Incremental Relaxation Algorithm (IR) }   
	\label{increamentalRelaxation}   
	\begin{algorithmic}[1] %"1" represents that it will show number in each row  
		\REQUIRE  %Input  
		a driver set $D$, an unserved rider request $r$, waiting constraint step \waitrelax, detour constraint step \detourrelax, maximal iteration time \iteration
		\ENSURE  %Output  
		return a suitable driver $d$
		\STATE \augdistance$\leftarrow 0$, \optaugdistance$\leftarrow\infty$, $d^*\leftarrow NIL$, \optntripschedule$\leftarrow NIL$, $w^\prime \leftarrow w$, $\theta^\prime \leftarrow \theta$, \unscanneddrivers$\leftarrow D$, \scanneddrivers$\leftarrow\emptyset$, $it \leftarrow 1$
		\FOR {$d \in$ \unscanneddrivers}
		\IF{ \dist($d$,$r$) $\leq w^\prime$ } 
		\STATE \unscanneddrivers$.pop(d)$, \scanneddrivers$.push(d)$ 		\COMMENT {Initialize \unscanneddrivers \xspace and \scanneddrivers \xspace}
		\STATE initialize $at$, $lt$, $sl$, and $cp$ using Eq. \ref{equ:at}-Eq. \ref{equ:cp}
		\ENDIF
		\ENDFOR
		\WHILE{$it\leq$ \iteration}
		\IF[Relax \detour] {($it$+1)\%2}	
		\STATE $\theta^\prime \leftarrow \theta^\prime$+\detourrelax	
		\FOR {$d \in$ \scanneddrivers}
		\STATE Algorithm \ref{relaxationbaseline} lines \ref{ba:for:for:start}-\ref{ba:for:for:for:update}
		\ENDFOR 
		\IF{$d^* \nleftarrow NIL$}
		\BREAK
		\ENDIF		
		\STATE update \sarr[$d.id$]
		\ELSE[Relax \wait]																
		\STATE $w^\prime \leftarrow w^\prime$+\waitrelax				
		\FOR {$d \in$ \unscanneddrivers}
		\IF {\dist($d$,$r$) $\leq w^\prime$}		
		\STATE initialize $at$, $lt$, $sl$, and $cp$ using Eq. \ref{equ:at}-Eq. \ref{equ:cp}	
		\STATE Algorithm \ref{relaxationbaseline} lines \ref{ba:for:for:start}-\ref{ba:for:for:for:update}		
		\IF{$d^* \nleftarrow NIL$}
		\BREAK
		\ENDIF		
		\STATE \unscanneddrivers$.pop(d)$, \scanneddrivers$.push(d)$				
		\STATE update \darr[$d.id$]
		\ENDIF
		\ENDFOR   		
		\ENDIF                                                  
		\ENDWHILE
		\RETURN $d^*$
	\end{algorithmic}  
\end{algorithm} 
\end{smaller}






==> sec7-divideconquer.tex <==
\section{Divide-and-Conquer Algorithm}\label{sec:dc}
As we know, given a bipartite graph from a set of drivers $D$ and a set of riders $R$, the size of all possible driver-and-rider assignments is exponential ($|D|^{|R|}$). By utilizing divide-and-conquer approach, the problem space can be dramatically reduced. 

The divide-and-conquer approach follows the idea of grouping both the drivers and riders. The main framework (Algo. \ref{dc:main}) includes three stages: (i) recursively divide the MDRTW problem into two smaller subproblems; (ii) solve two subproblems individually; (iii) merge the answers of two subproblems. In stage ii, we can use greedy algorithm to get an approximate result; In stage iii, we can directly merge the answers from each subgraph to form the final result because there is no overlap riders among all the groups. 
So the main challenge is that how can we divide a bilateral graph into two smaller subgraphs in stage i. 

\input{alg-divideconquer.tex}


\subsection{Divide the bipartite graph}
We first need to iteratively divide the whole graph into two subgraphs such that there are few drivers shared by these two subgraphs simultaneously. 

Since a rider can only be served by one driver nearby, which implies we only need to check partial driver candidates rather than all the drivers. Hence, we borrow the idea of ``quadtree''. We divide the riders recursively based on their locations on road network until the number of remaining riders is less than a threshold $\gamma$ such that it can be solved directly (Algo. \ref{dc:main} line \ref{dc:if}). Then we could obtain $m$ groups of riders: $R_1$, $R_2$, ..., $R_m$. For riders in each group, we consider the drivers which satisfy the waiting time constraint as candidates. Therefore, the result after partitioning the bipartite graph is ($D_1$,$R_1$), ($D_2$,$R_2$), ..., ($D_m$,$R_m$), where $R_1\cap R_2\cap...\cap R_m=\emptyset$, $R_1\cup R_2\cup...\cup R_m=R$, and $D_1\cup D_2\cup...\cup D_m \subseteq D$. Note that there may exist $D_i \cap D_j \neq \emptyset$ ($i \neq j$). 

\subsection{Merge the answers of the subproblems} 






==> sec7-samplingalgorithm.tex <==
\section{Sampling Algorithm}\label{sec:sa}
Since each rider can be only assigned to one driver, we can select one of 


==> sec8-relaxation.tex <==
\section{Rider request relaxation}\label{sec:relaxation}

\textbf{Motivation. }Existing work on ridesharing often define some hard constraints given by riders. If a rider is served successfully, his corresponding defined constraints must be met. 
However, it is possible that most riders can not be served by any driver because their prescribed constraint thresholds are intractable to be satisfied: (1) the waiting time constraint \wait is improperly specified by the rider for lack of the real road condition information; (2) the detour constraint \detour confines more riders' sharing paticipation.  

\textbf{Query relaxation mechanism. }In order to win back an unserved rider, the ridesharing system may (1) recommend the rider to prolong \wait such that some distant drivers can be added into the candidate set; (2) suggest the rider to lengthen \detour such that it allows to share a ride with more other riders on its way to the destination; (3) enlarge both \wait and \detour simultaneously. 

When we relax the constraints of an unserved rider, there are two rules to follow: (1) The relaxation mechanism is only applied into the current unserved rider, while the constraints by any served rider $r_s$ ($r_s \in$ \sriders) are maintained invariable owing to users' experience. (2) For any two unserved riders $r_u$ and $r_u^{\prime}$ ($r_u$, $r_u^{\prime} \in$ \uriders), their relaxation behaviors are neither relied on nor influenced by each other. 

\subsection{Baseline}

\input{alg-relaxationbaseline.tex}

\textbf{Algorithm sketch. }A straightforward solution is by brute force, which has the following main steps: 
(1) firstly, we compute the maximal relaxed waiting time constraint $w^\prime$ and detour constraint $\theta^\prime$ (line \ref{ba:initial}), which are considered as the limit of endurance riders could reach; 
(2) for each driver candidate, it enumerates all the possible insertion positions for both the source point \source and destination point \des; 
(3) for each possible insertion position pair $<$$i,j$$>$, check whether it violates the constraints of the following points in the trip schedule; 
(4) if there exist multiple driver choices, then return the one with the smallest augmented travel distance and update the corresponding trip schedule.
The algorithm is illustrated in Algo. \ref{relaxationbaseline}. 

\textbf{Time complexity analysis. }For each driver, suppose that $n$=$|d.tr|$, then traversing all the possible insertion pairs $<$$i,j$$>$ takes $O(n^2)$ time. For each new generated trip schedule \optntripschedule, we need to validate whether it will violate the constraints of the following points (line \ref{ba:for:for:if} or line \ref{ba:for:for:for:if}), which takes $O(1)$ time. Then update a driver candidate $d$ with smaller \augdistance \xspace than currently found. Hence, the total time complexity is $O(|D|n^2)$.
\subsection{Incremental Relaxation}

\input{alg-relaxationopt.tex}

\textbf{Algorithm sketch. }An incremental relaxation method aims to find a suitable driver by incrementally relaxing two constraint conditions \wait and \detour respectively, which has the following steps: (1) relax \detour by increasing \detourrelax. If it succeeds, then terminate the algorithm; (2) If it fails in the first step, then relax \wait by increasing \waitrelax; (3) If it still fails in the second step, then go the step (1) and proceed the relaxation operations repeatly until a driver which can serve is found or the algorithm reaches the maximal iteration time \iteration. Here, relaxing \wait could increase the number of driver candidates, while relaxing \detour indicates for a specific driver more updated trip schedules after a new rider insertion may be generated. 

==> tbl-dataset.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\caption{ Statistics of datasets. }
\centering
\begin{tabular}{|c|c|c|c|c|}
	\hline
	Dataset  & \#Vertices & \#Edges   & \#Requests & Time           \\ \hline
	Shanghai & 122,319    & 188,426   & 432,327    & May 29, 2009   \\ \hline
	Chengdu  & 287,656    &    & 259,406    & Nov 18, 2016   \\ \hline
	%NYC      & 807,795    & 2,100,632 & 517,100    & Apr 09, 2016 \\ \hline
\end{tabular}
\label{table:dataset}
\end{table}


